The VMC survey -- XLV. Proper motion of the outer LMC and the impact of the SMC

The Large Magellanic Cloud (LMC) is the most luminous satellite galaxy of the Milky Way and owing to its companion, the Small Magellanic Cloud (SMC), represents an excellent laboratory to study the interaction of dwarf galaxies. The aim of this study is to investigate the kinematics of the outer regions of the LMC by using stellar proper motions to understand the impact of interactions, e.g. with the SMC about 250 Myr ago. {We calculate proper motions using multi-epoch $K_\mathrm{s}$-band images from the VISTA survey of the Magellanic Clouds system (VMC). Observations span a time baseline of 2$-$5 yr. We combine the VMC data with data from the Gaia early Data Release 3 and introduce a new method to distinguish between Magellanic and Milky Way stars based on a machine learning algorithm. This new technique enables a larger and cleaner sample selection of fainter sources as it reaches below the red clump of the LMC. We investigate the impact of the SMC on the rotational field of the LMC and find hints of stripped SMC debris. The south east region of the LMC shows a slow rotational speed compared to the overall rotation. $N$-body simulations suggest that this could be caused by a fraction of stripped SMC stars, located in that particular region, that move opposite to the expected rotation.

==> figures/LMC_rotaion_VMC.tex <==
%-------------------------------------------------------------
%                 A figure as large as the width of the column
%-------------------------------------------------------------
   \begin{figure}
   \centering
   \includegraphics[width=\hsize]{figures/LMC_rotaion_VMC.png}
      \caption{Same as Fig.~\ref{LMC_rotaion_GaiaDR2} but for VMC proper motions.
              }
         \label{LMC_rotaion_VMC}
   \end{figure}
%

==> figures/classifier.tex <==
\begin{figure*}
   \centering
   \includegraphics[width=1.0\textwidth]{figures/classifier.png}
   
   \caption{ (Left) VMC proper motion distribution in right ascension and declination of classified sources indicating the Gaia DR2 proper motions of training sample (black), VMC proper motions classified as LMC stars (yellow) and Milky Way foreground sources (Blue). CMDs of the training sample in $Gaia$ magnitudes (Centre left) and VMC magnitudes (centre right) with the addition of the classified sources and their distribution in Gaia DR2 parallaxes (Right).}
    \label{classifier}% 
    \end{figure*}

==> figures/vmc_gaia_comparison.tex <==
%-------------------------------------------------------------
%                 A figure as large as the width of the column
%-------------------------------------------------------------
%additional plots
   \begin{figure}
   \centering
   \includegraphics[width=\hsize]{figures/diff_reflex_motion_pmra.png}
   \includegraphics[width=\hsize]{figures/diff_reflex_motion_pmdec.png}
      \caption{Difference between the effect of the solar reflex motion in the \textbf{Gaia} EDR3 mock catalogue and as measured with the data across the LMC on the proper motion components: $\mu_\alpha$cos$(\delta$) (top) and $\mu_\delta$ (bottom).}
         \label{reflex_motion}
   \end{figure}
%

==> tables/pm_table_VMC.tex <==
   %TableSH
    \begin{table}[]
    \caption{VMC proper motions of the outer LMC resulting from a SVM selection.}
    \label{pm_table_VMC}
    \begin{tabular}{cccccc}
    \hline\hline
    Bin &  d\tablefootmark{*}& stars   & $\mu_{\alpha}\cos{\delta}$     & $\mu_{\delta}$ & v$_\phi$\tablefootmark{**}   \\
        &  (deg)                     & & (mas~yr$^{-1}$) & (mas~yr$^{-1}$)&(km~s$^{-1}$) \\
    \hline
    1 & 3.70 &  297 & 1.97$\pm$0.08 & -0.46$\pm$0.16 &  82.5 \\
    ... & ... &  ... & ... & ... & ... \\
    1004 & 5.64 &  253 & 1.86$\pm$0.05 & -0.51$\pm$0.23 &  95.7 \\

    \hline
    \end{tabular}\\
    \tablefoottext{*}{Angular distance to the LMC centre.}\\
    \tablefoottext{**}{in respect to LMC centre}
    \end{table}
